Locally Estimating Core Numbers

Graphs are a powerful way to model interactions and relationships in data from a wide variety of application domains. In this setting, entities represented by vertices at the "center" of the graph are often more important than those associated with vertices on the "fringes". For example, central nodes tend to be more critical in the spread of information or disease and play an important role in clustering/community formation. Identifying such "core" vertices has recently received additional attention in the context of {\em network experiments}, which analyze the response when a random subset of vertices are exposed to a treatment (e.g. inoculation, free product samples, etc). Specifically, the likelihood of having many central vertices in any exposure subset can have a significant impact on the experiment. We focus on using $k$-cores and core numbers to measure the extent to which a vertex is central in a graph. Existing algorithms for computing the core number of a vertex require the entire graph as input, an unrealistic scenario in many real world applications. Moreover, in the context of network experiments, the subgraph induced by the treated vertices is only known in a probabilistic sense. We introduce a new method for estimating the core number based only on the properties of the graph within a region of radius $\delta$ around the vertex, and prove an asymptotic error bound of our estimator on random graphs. Further, we empirically validate the accuracy of our estimator for small values of $\delta$ on a representative corpus of real data sets. Finally, we evaluate the impact of improved local estimation on an open problem in network experimentation posed by Ugander et al.

==> sections/random_proof.tex <==
\begin{algorithm} 
\caption{Random Graph Generation from a given $k$-shell distribution\label{alg:random_generator}
}
\begin{algorithmic}[1]
	\STATE {\textsc{input}}:  $c_1,\dots ,c_D$, the number of vertices in graph $G_{real}$ with core number $1\dots D$
	\STATE {\textsc{output}}:  Random graph $G_{synth}$ with the same core number distribution as $G_{real}$
	\STATE $G_{synth} \leftarrow (V=\emptyset,E=\emptyset)$
	\FOR{$i \in \{D\dots1\}$} \label{alg:random_generator:outer_for}
		\STATE $V_i \leftarrow $ set of new vertices of size $c_i$
		\STATE $V \leftarrow V\cup V_i$
		\FOR{$v\in V_i$} \label{alg:random_generator:vertex}
			\IF{$d(v)<i$}
				\STATE $U \leftarrow $ set of $i-d(v)$ randomly selected vertices not adjacent to $v$
				\FOR{$u\in U$}\label{alg:random_generator:edge_addition_start}
					\STATE $E\leftarrow E \cup (u,v)$ 
				\ENDFOR\label{alg:random_generator:edge_addition_end}
			\ENDIF
		\ENDFOR
	\ENDFOR
	\RETURN $G_{synth}$
\end{algorithmic}
\end{algorithm}
The novel graph generator starts with an empty graph and iteratively grows from the deepest shell to the shallowest.  The vertex set $V_i$ contains the vertices intended to be placed in the $i$-shell of $G_{synth}$.  When $V_i$ is added to the graph, edges are added until all vertices have a minimum degree $i$.  We will formally prove that the output of Algorithm \ref{alg:random_generator} is always a graph with a shell distribution matching its input.
\begin{lemma} \label{thm:k_int}
Let $k_{int}(v)$ be the value of $i$ for which $v\in V_i$ in Algorithm \ref{alg:random_generator}.  $\forall v\in V$, $k_{int}(v)=k(v)$.
\end{lemma}
\begin{proof}
We prove by demonstrating that $k_{int}(v)\leq k(v)$ and $k(v)\geq k_{int}(v)$ are simultaneously true.
At each iteration of the outer \texttt{for} loop (line \ref{alg:random_generator:outer_for}), we attempt to produce an $i$-core in $G_{synth}$ of the same size as that of $G_{real}$.  Thus, $\forall v\in V_i$, $k_{int}(v) = i$.  Edges are added until each vertex has degree at least $i$, so we are guaranteed that if $v$ was added in the most recent iteration, then $k(v)\geq k_{int}(v)$.
\\
We prove $k(v)\leq k_{int}(v)$ by induction on the addition of edges in lines \ref{alg:random_generator:edge_addition_start}-\ref{alg:random_generator:edge_addition_end}.  Before any edges are added, $\forall v \in V$, $d(v)=k(v)=0\leq k_{int}(v)$.  Let $v$ be the $j$th vertex to be considered at line \ref{alg:random_generator:vertex} and let $E_j$ be the set of $(u,v)$ edges to be added.  Assume that prior to adding $E_j$ to $E$, $\forall x\in V$, $k_{int}(x)\geq k(x)$.  After adding $E_j$ to $E$, $d(v)=i$.  Since $k(v)\leq d(v)$ and $k_{int}(v) = i$, $k_{int}(v)\geq k(v)$.
\\
Suppose $\exists v'\in V | v'\neq v$ such that adding $E_j$ to $E$ causes $k(v')> k_{int}(v') $.  Because all vertices already added to $G_{synth}$ have $k_{int}\geq i$, $k(v')> k(v)$ after $E_j$ is added.  This means that the $k(v')$-core does not include $v$, so any of the edges in $E_j$ are not part of the subgraph induced on the $k(v')$-core.  Therefore, $k(v')$ was already greater than $k_{int}(v')$ prior to the addition of $E_j$, which is a contradiction.  Hence, $\forall x\in V$, $k_{int}(x)\geq k(x)$ remains true after adding $E_j$. \\
Since $k_{int}(v)\geq k(v) \geq k_{int}(v)$, $k_{int}(v)=k(v)$.
\end{proof}

%\subsubsection{Edge Preservation}
%Suppose in Algorithm \ref{alg:random_generator} we have already generated cores $D$ through $D-j+1$ in $G$.  Suppose in generating the $j$-core, all vertices with core number $j$ form one $j$-regular component that is disconnected from $G$.  Call this graph $H$.  Suppose also that in generating the $j$-core, the vertices with core number $j$ form an independent set.  That is to say, all edges are between vertices with core number $j$ and core number greater than $j$.  Call this graph $H'$.  Therefore $|E(H)| = |E(G)| + jc_j/2$ and $E(H') = |E(G)| + jc_j$.  Since two outcomes of generating a core can have differing number of edges, Algorithm \ref{alg:random_generator} does not preserve edges from the original graph.
%\subsubsection{Uniformity}
%Algorithm \ref{alg:random_generator} probably does not sample uniformly at random across all graphs with a given core sequence.  When adding edges to a vertex $v$, edges connecting $v$ to a vertex in the same core are selected with some probability $p$, while edges to vertices from a greater core are selected with probability $1-p$.  Then the distribution of graphs generated should roughly follow a binominal distribution, but they don't.  (?)

